Accelerating science with human versus alien artificial intelligences

Data-driven artificial intelligence models fed with published scientific findings have been used to create powerful prediction engines for scientific and technological advance, such as the discovery of novel materials with desired properties and the targeted invention of new therapies and vaccines. These AI approaches typically ignore the distribution of human prediction engines -- scientists and inventor -- who continuously alter the landscape of discovery and invention. As a result, AI hypotheses are designed to substitute for human experts, failing to complement them for punctuated collective advance. Here we show that incorporating the distribution of human expertise into self-supervised models by training on inferences cognitively available to experts dramatically improves AI prediction of future human discoveries and inventions. Including expert-awareness into models that propose (a) valuable energy-relevant materials increases the precision of materials predictions by ~100%, (b) repurposing thousands of drugs to treat new diseases increases precision by 43%, and (c) COVID-19 vaccine candidates examined in clinical trials by 260%. These models succeed by predicting human predictions and the scientists who will make them. By tuning AI to avoid the crowd, however, it generates scientifically promising "alien" hypotheses unlikely to be imagined or pursued without intervention, not only accelerating but punctuating scientific advance. By identifying and correcting for collective human bias, these models also suggest opportunities to improve human prediction by reformulating science education for discovery.

==> TikzScripts/papers/paper_1.tex <==

\newsavebox\paperone


\begin{lrbox}{\paperone}
\node at (0,0) {\includegraphics[width=45pt]{Figures/paper_symbols/blank.png}};
\draw[fill=blue, blue](.3,-.5) circle (3pt);

\node at (0,.3) {$\Diamond$, $\square$, \whitecircle};
\end{lrbox}



==> TikzScripts/papers/paper_2.tex <==

\newsavebox\papertwo


\begin{lrbox}{\papertwo}
    \node at (0,0) {\includegraphics[width=45pt]{Figures/paper_symbols/blank.png}};
    \draw[fill=blue, blue](-.2,-.25) circle (3pt);
    \filldraw[fill=blue,draw=blue] (.3,-.5) rectangle ++(5pt,5pt);
    
    \node at (0,.3) {$\vartriangle$, $\triangledown$};
\end{lrbox}



==> TikzScripts/papers/paper_3.tex <==

\newsavebox\paperthree


\begin{lrbox}{\paperthree}
\node at (0,0) {\includegraphics[width=45pt]{Figures/paper_symbols/blank.png}};
\draw[fill=red, red](-.3,-.5) circle (3pt);
\draw[fill=red, red](.4,.77) circle (3pt);

\node at (0,.3) {$\Diamond$, $\rhd$};
\node at (.4,-.5) {\scalebox{1.5}{\bluetriangle}};
\node at (.15,-.2) {\scalebox{1.5}{\bluedowntriangle}};
\end{lrbox}


